Voxtral

We present Voxtral Mini and Voxtral Small, two multimodal audio chat models. Voxtral is trained to comprehend both spoken audio and text documents, achieving state-of-the-art performance across a diverse range of audio benchmarks, while preserving strong text capabilities. Voxtral Small outperforms a number of closed-source models, while being small enough to run locally. A 32K context window enables the model to handle audio files up to 40 minutes in duration and long multi-turn conversations. We also contribute three benchmarks for evaluating speech understanding models on knowledge and trivia. Both Voxtral models are released under Apache 2.0 license.

==> tables.tex <==
\begin{table}[h]
\centering
\caption{\textbf{Speech Recognition Benchmarks.} Macro-average WER results across tasks. Voxtral Small outperforms all open and closed-source models on English Short-Form, MCV and MLS.} \label{tab:asr-avg}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
\textbf{Model}          & \multicolumn{1}{l}{\textbf{En Short}} & \multicolumn{1}{l}{\textbf{En Long}} & \multicolumn{1}{l}{\textbf{MCV}} & \multicolumn{1}{l}{\textbf{FLEURS}} & \multicolumn{1}{l}{\textbf{MLS}} \\ \midrule
Whisper large-v3        & 7.69                               & 11.48                             & 14.09                         & 8.29                             & 6.78                          \\
GPT-4o mini Transcribe  & 8.85                               & 11.18                             & 12.29                         & 5.72                             & 6.58                          \\
Gemini 2.5 Flash        & 8.04                               & 9.45                              & 8.77                          & 7.04                             & 7.36                          \\
Scribe                  & 6.41                               & \textbf{8.27}                      & 5.87                          & \textbf{4.91}                     & 15.06                         \\ \midrule
Voxtral Mini            & 6.79                               & 10.73                             & 7.83                          & 7.08                             & 7.60                          \\
Voxtral Mini Transcribe & 6.43                               & 10.85                             & 6.32                          & 5.54                             & 6.29                          \\
Voxtral Small           & \textbf{6.31}                       & 11.02                             & \textbf{5.65}                  & 5.11                             & \textbf{6.11}                  \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{\textbf{FLEURS Translation.} BLEU scores for source/target language pairs on the FLEURS Translation benchmark. Voxtral Small achieves state-of-the-art for every pair of languages. Whisper only supports X $\rightarrow$ en translation.} \label{tab:fleurs-translation}
\begin{tabular}{@{}lrrrrrrrr@{}}
\toprule
\textbf{Model}                   & \rotatebox{90}{en $\rightarrow$ de} & \rotatebox{90}{en $\rightarrow$ es} & \rotatebox{90}{en $\rightarrow$ fr} & \rotatebox{90}{en $\rightarrow$ it} & \rotatebox{90}{de $\rightarrow$ en} & \rotatebox{90}{es $\rightarrow$ en} & \rotatebox{90}{fr $\rightarrow$ en} & \rotatebox{90}{it $\rightarrow$ en} \\ 
\midrule
Whisper large-v3        &         -                            &    -                                 &                  -                   &            -                         & 46.1                               & 34.9                               & 43.0                               & 35.7                               \\
GPT-4o mini Audio       & 44.5                                & 36.5                                & 52.7                                & 37.3                                & 51.8                               & 41.6                               & 48.2                               & 41.5                               \\
Gemini 2.5 Flash         & 44.6                                & 36.3                                & 53.9                                & 37.3                                & 39.4                               & 32.9                               & 42.0                               & 31.8                               \\
Voxtral Mini            & 38.4                                & 34.9                                & 49.7                                & 34.2                                & 49.6                               & 41.1                               & 48.2                               & 41.4                               \\
Voxtral Small           & \textbf{47.0}                       & \textbf{39.9}                       & \textbf{57.3}                       & \textbf{39.9}                       & \textbf{56.6}                      & \textbf{46.3}                      & \textbf{54.2}                      & \textbf{46.8}                      \\ 
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{\textbf{speech understanding Benchmarks.} We report the accuracy across three speech understanding benchmarks, and four synthesized subsets of text benchmarks, denoted with\textsuperscript{*}. Voxtral Small is competitive with closed-source models, surpassing GPT-4o mini Audio on three of the seven benchmarks.} \label{tab:au}
\begin{footnotesize}

\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
\textbf{Model}    & \textbf{Llama QA} & \textbf{Openbook QA} & \textbf{MMLU\textsuperscript{*}} & \textbf{MMAU\textsuperscript{*}} & \textbf{Trivia QA\textsuperscript{*}} & \textbf{GSM8k\textsuperscript{*}} & \textbf{AU Bench} \\ \midrule
GPT-4o mini Audio & \textbf{74.3}                     & 83.7                 & 72.6              & 63.4              & 83.7                   & 90.8               & 80.0                  \\
Gemini 2.5 Flash  & 66.3                     & \textbf{94.7}                 & \textbf{84.8}      & \textbf{64.3}     & \textbf{83.9}                   & \textbf{94.2}               & \textbf{88.6}                  \\
Voxtral Mini      & 54.3                     & 59.6                 & 47.6              & 57.1              & 54.9                   & 71.6               & 85.6                  \\
Voxtral Small     & 71.7                     & 88.4                 & 74.3              & 62.2              & 79.4                   & 89.7               & 86.6                  \\ \bottomrule
\end{tabular}
\end{footnotesize}
\end{table}

\begin{table}[H]
\centering
\caption{English speech recognition results by task.} \label{tab:asr-en}
\begin{tabular}{@{}l|rrrrrrr|rr@{}}
\toprule
Model                   & \rotatebox{90}{LibriSpeech Clean} & \rotatebox{90}{LibriSpeech Other} & \rotatebox{90}{GigaSpeech} & \rotatebox{90}{VoxPopuli} & \rotatebox{90}{SwitchBoard} & \rotatebox{90}{CHiME-4} & \rotatebox{90}{SPGISpeech} & \rotatebox{90}{Earnings-21 10m} & \rotatebox{90}{Earnings-22 10m} \\ \midrule
Whisper large-v3        & 1.84                                                 & 3.66                                                 & 11.60                                         & 9.58                                         & 13.14                                          & 10.88                                      & 3.15                                          & 9.88                                               & 13.07                                              \\
GPT4o mini Transcribe   & 1.92                                                 & 4.70                                                 & 14.80                                         & 7.34                                         & 17.31                                          & 11.35                                      & 4.51                                          & 10.09                                              & 12.27                                              \\
Gemini 2.5 Flash        & 2.97                                                 & 6.15                                                 & 10.99                                         & 7.84                                         & \textbf{9.57}                                  & 14.79                                      & 4.00                                          & 8.09                                               & 10.80                                              \\
ElevenLabs Scribe       & 1.80                                                 & 3.44                                                 & 10.52                                         & 6.95                                         & 10.62                                          & \textbf{8.35}                              & 3.16                                          & \textbf{7.39}                                      & \textbf{9.16}                                      \\ \midrule
Voxtral Mini            & 1.86                                                 & 4.04                                                 & 10.68                                         & 6.85                                         & 11.32                                          & 10.59                                      & 2.19                                          & 9.62                                               & 11.84                                              \\
Voxtral Mini Transcribe & 1.57                                                 & 3.21                                                 & \textbf{10.04}                                & 6.78                                         & 11.35                                          & 10.03                                      & 2.04                                          & 9.52                                               & 12.18                                              \\
Voxtral Small           & \textbf{1.53}                                        & \textbf{3.14}                                        & 10.27                                         & \textbf{6.62}                                & 11.09                                          & 9.64                                       & \textbf{1.89}                                 & 9.55                                               & 12.48                                              \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[H]
\centering
\caption{English speech recognition results by task. We report short-form scores for LibriSpeech Test Clean (LS-C), LibriSpeech Test Other (LS-O), GigaSpeech (GS), VoxPopuli (VP), SwitchBoard (SB), CHiME-4 (C-4) and SPGISPeech (SPGI). We report long-form scores for Earnings-21 10m (E21 10m) and Earnings-22 10m (E22 10m).} \label{tab:asr-en-alt}
\begin{tabular}{@{}l|rrrrrrr|rr@{}}
\toprule
Model                   & \multicolumn{1}{c}{LS-C} & \multicolumn{1}{c}{LS-O} & \multicolumn{1}{c}{GS} & \multicolumn{1}{c}{VP} & \multicolumn{1}{c}{SB} & \multicolumn{1}{c}{C-4} & \multicolumn{1}{c|}{SPGI} & \multicolumn{1}{c}{E21 10m} & \multicolumn{1}{c}{E22 10m} \\ \midrule
Whisper large-v3        & 1.84                                                 & 3.66                                                 & 11.60                                         & 9.58                                         & 13.14                                          & 10.88                                      & 3.15                                          & 9.88                                               & 13.07                                              \\
GPT4o mini Transcribe   & 1.92                                                 & 4.70                                                 & 14.80                                         & 7.34                                         & 17.31                                          & 11.35                                      & 4.51                                          & 10.09                                              & 12.27                                              \\
Gemini 2.5 Flash        & 2.97                                                 & 6.15                                                 & 10.99                                         & 7.84                                         & \textbf{9.57}                                  & 14.79                                      & 4.00                                          & 8.09                                               & 10.80                                              \\
ElevenLabs Scribe       & 1.80                                                 & 3.44                                                 & 10.52                                         & 6.95                                         & 10.62                                          & \textbf{8.35}                              & 3.16                                          & \textbf{7.39}                                      & \textbf{9.16}                                      \\ \midrule
Voxtral Mini            & 1.86                                                 & 4.04                                                 & 10.68                                         & 6.85                                         & 11.32                                          & 10.59                                      & 2.19                                          & 9.62                                               & 11.84                                              \\
Voxtral Mini Transcribe & 1.57                                                 & 3.21                                                 & \textbf{10.04}                                & 6.78                                         & 11.35                                          & 10.03                                      & 2.04                                          & 9.52                                               & 12.18                                              \\
Voxtral Small           & \textbf{1.53}                                        & \textbf{3.14}                                        & 10.27                                         & \textbf{6.62}                                & 11.09                                          & 9.64                                       & \textbf{1.89}                                 & 9.55                                               & 12.48                                              \\ \bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{Per-language WER scores for FLEURS.}
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
Model                   & \rotatebox{90}{Arabic} & \rotatebox{90}{Dutch} & \rotatebox{90}{English} & \rotatebox{90}{French} & \rotatebox{90}{German} & \rotatebox{90}{Hindi} & \rotatebox{90}{Italian} & \rotatebox{90}{Portuguese} & \rotatebox{90}{Spanish} \\ \midrule
Whisper large-v3        & 15.44                   & 5.87                   & 4.00                     & 5.55                    & 5.46                    & 28.87                  & 2.71                     & 3.90                         & 2.81                      \\
GPT-4o mini Transcribe  & 14.02                   & 5.54                   & \textbf{3.19}            & 4.51                    & 3.76                    & 12.36                  & 2.02                     & \textbf{3.54}                & \textbf{2.58}             \\
Gemini 2.5 Flash        & 25.25                   & 6.20                   & 4.64                     & 6.17                    & 4.74                    & 6.76                   & 2.21                     & 4.23                         & 3.17                      \\
Scribe                  & \textbf{11.58}          & \textbf{4.63}          & 3.29                     & 5.07                    & 4.78                    & \textbf{5.67}          & \textbf{1.48}            & 4.50                         & 3.13                      \\
Voxtral Mini            & 25.40                   & 6.27                   & 3.77                     & 4.87                    & 4.40                    & 9.26                   & 2.51                     & 3.76                         & 3.52                      \\
Voxtral Mini Transcribe & 14.64                   & 4.89                   & 3.61                     & 4.22                    & 3.54                    & 10.32                  & 2.31                     & 3.57                         & 2.75                      \\
Voxtral Small           & 13.44                   & 4.94                   & 3.35                     & \textbf{4.03}           & \textbf{3.38}           & 7.69                   & 2.62                     & 3.79                         & 2.72                      \\ \bottomrule
\end{tabular}
\end{table}



\begin{table}[h]
\centering
\caption{Per-language WER scores for MCV. For fairness, we omit Arabic from the macro-average in Table \ref{tab:asr-avg}, since all models score in excess of 45\%.}
\begin{tabular}{@{}lrrrrrrrrr@{}}
\toprule
Model                   & \rotatebox{90}{Arabic} & \rotatebox{90}{Dutch} & \rotatebox{90}{English} & \rotatebox{90}{French} & \rotatebox{90}{German} & \rotatebox{90}{Hindi} & \rotatebox{90}{Italian} & \rotatebox{90}{Portuguese} & \rotatebox{90}{Spanish} \\ \midrule
Whisper large-v3        & 50.58                   & 5.83                   & 22.91                    & 11.33                   & 6.25                    & 46.75                  & 6.81                     & 7.17                         & 5.66                      \\
GPT-4o mini Transcribe  & 51.68                   & 6.47                   & 13.15                    & 10.75                   & 6.72                    & 39.06                  & 6.16                     & 9.95                         & 6.10                      \\
Gemini 2.5 Flash        & 53.62                   & 5.73                   & 12.31                    & 11.86                   & 7.25                    & 11.09                  & 6.64                     & 9.42                         & 5.88                      \\
Scribe                  & \textbf{47.03}          & \textbf{2.38}          & \textbf{6.59}            & \textbf{5.44}           & \textbf{3.52}           & 17.29                  & \textbf{2.99}            & \textbf{5.46}                & \textbf{3.27}             \\
Voxtral Mini            & 63.98                   & 6.03                   & 10.22                    & 8.92                    & 6.07                    & 12.74                  & 5.91                     & 7.76                         & 4.98                      \\
Voxtral Mini Transcribe & 62.01                   & 4.71                   & 8.25                     & 7.29                    & 4.85                    & 10.42                  & 4.37                     & 6.70                         & 3.96                      \\
Voxtral Small           & 61.97                   & 3.98                   & 8.58                     & 6.18                    & 3.74                    & \textbf{9.01}          & 3.96                     & 6.43                         & 3.31                      \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Per‐language WER scores for MLS.}
\begin{tabular}{@{}lrrrrrr@{}}
\toprule
Model                   & \rotatebox{90}{Dutch}   & \rotatebox{90}{French}  & \rotatebox{90}{German}   & \rotatebox{90}{Italian}  & \rotatebox{90}{Portuguese} & \rotatebox{90}{Spanish}  \\ 
\midrule
Whisper large-v3        &  9.19 &  5.09 &  5.72 &   9.78 &     7.03 &   3.89 \\
GPT-4o mini Transcribe  &  8.62 &  4.77 & \textbf{5.44} &  10.68 &     5.67 &   4.28 \\
Gemini 2.5 Flash        & \textbf{8.33} &  6.82 &  6.52 &  10.97 &     7.14 &   4.39 \\
Scribe                  & 38.01 &  5.80 &  9.81 &  12.38 &    15.40 &   8.97 \\
Voxtral Mini            & 10.09 &  5.28 &  7.09 &  11.30 &     6.72 &   5.12 \\
Voxtral Mini Transcribe &  9.63 &  4.14 &  5.64 &   9.28 & \textbf{5.17} &   3.87 \\
Voxtral Small           &  9.43 & \textbf{3.73} &  5.57 & \textbf{8.44} &     5.85 & \textbf{3.62} \\ 
\bottomrule
\end{tabular}
\end{table}

% WER figures

\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{results/all_en.png}
    \caption{English speech recognition results by task.} \label{fig:asr-en}
\end{figure}

Figures \ref{fig:fleurs}, \ref{fig:mcv} and \ref{fig:mls} show the per-language breakdown of WER scores for the FLEURS, Mozilla Common Voice and Multilingual LibriSpeech \citep{pratap2020mls} benchmarks, respectively.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{results/fleurs.png}
    \caption{Per-language WER scores for FLEURS.} \label{fig:fleurs}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{results/mcv.png}
    \caption{Per-language WER scores for Mozilla Common Voice 15.1.} \label{fig:mcv}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.85\textwidth]{results/mls.png}
    \caption{Per-language WER scores for Multilingual LibriSpeech.} \label{fig:mls}
\end{figure}
